Protecting User Privacy: An Approach for Untraceable Web Browsing History and Unambiguous User Profiles

The overturning of the Internet Privacy Rules by the Federal Communications Commissions (FCC) in late March 2017 allows Internet Service Providers (ISPs) to collect, share and sell their customers' Web browsing data without their consent. With third-party trackers embedded on Web pages, this new rule has put user privacy under more risk. The need arises for users on their own to protect their Web browsing history from any potential adversaries. Although some available solutions such as Tor, VPN, and HTTPS can help users conceal their online activities, their use can also significantly hamper personalized online services, i.e., degraded utility. In this paper, we design an effective Web browsing history anonymization scheme, PBooster, aiming to protect users' privacy while retaining the utility of their Web browsing history. The proposed model pollutes users' Web browsing history by automatically inferring how many and what links should be added to the history while addressing the utility-privacy trade-off challenge. We conduct experiments to validate the quality of the manipulated Web browsing history and examine the robustness of the proposed approach for user privacy protection.

==> npc.tex <==
%\begin{theorem}
%	\label{theo:NPC}
%	The optimization problem in Eq.\ref{optimization} is NP-complete.
%\end{theorem}

%We first demonstrate Proposition~\ref{prop:NIP} which enables us to prove Theorem~\ref{theo:NPC} later.

%\begin{prop}
%	\label{prop:NIP}
%	The optimization problem in Eq.\ref{optimization} is a non-linear integer programming problem with linear constraints.
%\end{prop}

%\begin{proof}
Given $\lambda \in [0,1]$ and topic count vector $c_u$, we can rewrite the optimization problem in Eq.\ref{optimization} as:
\begin{equation}
\label{eq:NIP}
\begin{split}
\underset{\hat{c}_u}{\argmaxG}  -\lambda(\sum_{j}\frac{\hat{c}_{uj}}{|\hat{H}^u|}\log&\frac{\hat{c}_{uj}}{|\hat{H}^u|}) +  (1-\lambda)\frac{\sum_jb_j\hat{c}_{uj}}{a\sqrt{\sum_j\hat{c}_{uj}^2}} \\
subject \; to \;  -\hat{c}_{uj} & \le -c_{uj} \;,  \hat{c}_{uj} \in \mathbb{N}^0\\
\end{split}
\end{equation}  
where $b_j = p_{uj}$, $a = ||p_{u}||$ are constant given user $u$ and $|\hat{H}^u|=\sum_j\hat{c}_{uj}$ is the size of browsing history after \textsc{PBooster} is applied.
%
This is a non-negative non-monotone submodular maximization problem, which is NP-hard as shown in~\cite{feige2011maximizing}.

%Eq.\ref{eq:NIP} matches the form of nonlinear integer programming~\cite{hemmecke2010nonlinear} with linear constraints.
%Then we show there exists a special case of Eq.\ref{eq:NIP} which is an integer linear programming problem.
%
%We define $\hat{d}_{uj} = \hat{c}_{uj}-c_{uj}$.
%
%By adding a constraint $\sum_{j=1}^m\hat{d}_{uj}^2=1$, and fixing $\lambda=0$, we can reduce Eq.\ref{eq:NIP} to:
%\begin{equation}
%\label{eq:ILP}
%\begin{split}
%\underset{\hat{d}_u}{\argmaxG}& \frac{\sum_jb_j\hat{d}_{uj}}{a\sqrt{C}} \\
%subject \; to \;
%& \sum_{j}\hat{d}_{uj} = 1 , \hat{d}_{uj}  \in \mathbb{N}^0\\
%\end{split}
%\end{equation}
%This is because $\sum_{j}\hat{d}_{uj} = 1$ is equivalent to $\sum_{j}\hat{d}_{uj}^2 = 1$ for $\hat{c}_{uj}  \in \mathbb{N}^0$.
%
%Eq.\ref{eq:ILP} is thus an integer linear programming problem which in known as NP-complete--3SAT can be easily reduced to it.
%
%This completes the proof of Theorem~\ref{theo:NPC}.
%\end{proof}

It is worth it to mention that the search space for the original problem (Eq.\ref{optimization}) is exponential to $N$ ($\mathcal{O}(m\times 2^N)$), where $N$ is the maximum of the number of links w.r.t. to a topic. Considering this fact, it can be expensive and even infeasible to search for the optimal solution.

